Reducing Hyperparameter Tuning Costs in ML, Vision and Language Model Training Pipelines via Memoization-Awareness

The training or fine-tuning of machine learning, vision, and language models is often implemented as a pipeline: a sequence of stages encompassing data preparation, model training and evaluation. In this paper, we exploit pipeline structures to reduce the cost of hyperparameter tuning for model training/fine-tuning, which is particularly valuable for language models given their high costs in GPU-days. We propose a "memoization-aware" Bayesian Optimization (BO) algorithm, EEIPU, that works in tandem with a pipeline caching system, allowing it to evaluate significantly more hyperparameter candidates per GPU-day than other tuning algorithms. The result is better-quality hyperparameters in the same amount of search time, or equivalently, reduced search time to reach the same hyperparameter quality. In our benchmarks on machine learning (model ensembles), vision (convolutional architecture) and language (T5 architecture) pipelines, we compare EEIPU against recent BO algorithms: EEIPU produces an average of $103\%$ more hyperparameter candidates (within the same budget), and increases the validation metric by an average of $108\%$ more than other algorithms (where the increase is measured starting from the end of warm-up iterations).

==> impact.tex <==


% In this section, we examine the impact of memoization on the optimization proces. Then, we will evaluate our choice to cache the top $5$ prefixes by comparing the impact of different caching values on the final objective value across a set of synthetic pipelines.



% \subsection{Ablation Experiments}
% \label{sec:ablations}

% The proposed EEIPU architecture is an elaborate expansion of the EI acquisition function, introducing multiple components and variables to achieve our objective. The choices of our added parameters---cost-cooling factor, Nº of top-performing configurations $Q$, $\epsilon$, number of cached prefixes per observation---, were based on ablation experiments that we ran on our set of synthetic and real experiments. Section~\ref{a:ablation} of the appendix defines the nature of the experiments we ran, a summary and visualization of our results, and the intuition explaining our chosen values and what they mean for the underlying BO process.

